The Compositional Structure of Bayesian Inference

Bayes' rule tells us how to invert a causal process in order to update our beliefs in light of new evidence. If the process is believed to have a complex compositional structure, we may observe that the inversion of the whole can be computed piecewise in terms of the component processes. We study the structure of this compositional rule, noting that it relates to the lens pattern in functional programming. Working in a suitably general axiomatic presentation of a category of Markov kernels, we see how we can think of Bayesian inversion as a particular instance of a state-dependent morphism in a fibred category. We discuss the compositional nature of this, formulated as a functor on the underlying category and explore how this can used for a more type-driven approach to statistical inference.

==> diag/binv-equiv-proof-2.tex <==
% https://varkor.github.io/tangle/?t=W1tbXV0sW1tbMCxbXV0sWzAsW11dLFswLFtdXSxbMCxbXV0sWzAsW11dLFswLFtdXSxbMCxbXV0sWzAsW11dXSxbWzAsW11dLFswLFtdXSxbMCxbXV0sWzIsWzJdXSxbMSxbMCwxLDAsMV1dLFsxLFswLDEsMCwxXV0sWzEsWzAsMSwwLDFdXSxbMSxbMCwxLDAsMV1dXSxbWzEsWzAsMSwwLDBdXSxbMSxbMCwxLDAsMV1dLFsxLFswLDEsMCwxXV0sWzEsWzEsMCwxLDFdXSxbMCxbXV0sWzAsW11dLFswLFtdXSxbMCxbXV1dLFtbMCxbXV0sWzAsW11dLFswLFtdXSxbMixbMV1dLFsxLFswLDEsMCwxXV0sWzEsWzAsMSwwLDFdXSxbMSxbMCwxLDAsMV1dLFsxLFswLDEsMCwxXV1dXSxbWzAsMiwyLjUsWyJmIiwxLDFdXSxbMCwwLjUsMi41LFsicCIsMCwxXV0sWzAsNSwxLjUsWyJoIiwxLDFdXSxbMCw2LjUsMS41LFsiIl1dLFswLDcuNSwxLjUsWyIiXV1dXQ==&c=F5A3A3,F5CCA3,F5F5A3,CCF5A3,A3F5A3,A3F5CC,A3F5F5,A3CCF5,A3A3F5,CCA3F5,F5A3F5,F5A3CC
\begin{tangle}{(8,4)}
	\tgBlank{(0,0)}{white}
	\tgBlank{(1,0)}{white}
	\tgBlank{(2,0)}{white}
	\tgBlank{(3,0)}{white}
	\tgBlank{(4,0)}{white}
	\tgBlank{(5,0)}{white}
	\tgBlank{(6,0)}{white}
	\tgBlank{(7,0)}{white}
	\tgBlank{(0,1)}{white}
	\tgBlank{(1,1)}{white}
	\tgBlank{(2,1)}{white}
	\tgBorderC{(3,1)}{1}{white}{white}
	\tgBorderA{(4,1)}{white}{white}{white}{white}
	\tgBorder{(4,1)}{0}{1}{0}{1}
	\tgBorderA{(5,1)}{white}{white}{white}{white}
	\tgBorder{(5,1)}{0}{1}{0}{1}
	\tgBorderA{(6,1)}{white}{white}{white}{white}
	\tgBorder{(6,1)}{0}{1}{0}{1}
	\tgBorderA{(7,1)}{white}{white}{white}{white}
	\tgBorder{(7,1)}{0}{1}{0}{1}
	\tgBorderA{(0,2)}{white}{white}{white}{white}
	\tgBorder{(0,2)}{0}{1}{0}{0}
	\tgBorderA{(1,2)}{white}{white}{white}{white}
	\tgBorder{(1,2)}{0}{1}{0}{1}
	\tgBorderA{(2,2)}{white}{white}{white}{white}
	\tgBorder{(2,2)}{0}{1}{0}{1}
	\tgBorderA{(3,2)}{white}{white}{white}{white}
	\tgBorder{(3,2)}{1}{0}{1}{1}
	\tgBlank{(4,2)}{white}
	\tgBlank{(5,2)}{white}
	\tgBlank{(6,2)}{white}
	\tgBlank{(7,2)}{white}
	\tgBlank{(0,3)}{white}
	\tgBlank{(1,3)}{white}
	\tgBlank{(2,3)}{white}
	\tgBorderC{(3,3)}{0}{white}{white}
	\tgBorderA{(4,3)}{white}{white}{white}{white}
	\tgBorder{(4,3)}{0}{1}{0}{1}
	\tgBorderA{(5,3)}{white}{white}{white}{white}
	\tgBorder{(5,3)}{0}{1}{0}{1}
	\tgBorderA{(6,3)}{white}{white}{white}{white}
	\tgBorder{(6,3)}{0}{1}{0}{1}
	\tgBorderA{(7,3)}{white}{white}{white}{white}
	\tgBorder{(7,3)}{0}{1}{0}{1}
	\tgCell[(1,1)]{(1.5,2)}{f}
	\tgCell[(0,1)]{(0,2)}{p}
	\tgCell[(1,1)]{(4.5,1)}{h}
	\tgRestr{(6,1)}{}
	\tgIncl{(7,1)}{}
\end{tangle}

==> diag/binv-equiv-proof-3.tex <==
% https://varkor.github.io/tangle/?t=W1tbXV0sW1tbMCxbXV0sWzIsWzJdXSxbMSxbMCwxLDAsMV1dLFsxLFswLDEsMCwxXV0sWzEsWzAsMSwwLDFdXSxbMSxbMCwxLDAsMV1dXSxbWzEsWzAsMSwwLDBdXSxbMSxbMSwwLDEsMV1dLFswLFtdXSxbMCxbXV0sWzAsW11dLFswLFtdXV0sW1swLFtdXSxbMixbMV1dLFsxLFswLDEsMCwxXV0sWzEsWzAsMSwwLDFdXSxbMSxbMCwxLDAsMV1dLFsxLFswLDEsMCwxXV1dLFtbMCxbXV0sWzAsW11dLFswLFtdXSxbMCxbXV0sWzAsW11dLFswLFtdXV1dLFtbMCw0LjUsMC41LFsiIl1dLFswLDUuNSwwLjUsWyIiXV0sWzAsMywyLjUsWyJmIiwxLDFdXSxbMCwwLjUsMS41LFsicCIsMCwxXV1dXQ==&c=F5A3A3,F5CCA3,F5F5A3,CCF5A3,A3F5A3,A3F5CC,A3F5F5,A3CCF5,A3A3F5,CCA3F5,F5A3F5,F5A3CC
\begin{tangle}{(6,4)}
	\tgBlank{(0,0)}{white}
	\tgBorderC{(1,0)}{1}{white}{white}
	\tgBorderA{(2,0)}{white}{white}{white}{white}
	\tgBorder{(2,0)}{0}{1}{0}{1}
	\tgBorderA{(3,0)}{white}{white}{white}{white}
	\tgBorder{(3,0)}{0}{1}{0}{1}
	\tgBorderA{(4,0)}{white}{white}{white}{white}
	\tgBorder{(4,0)}{0}{1}{0}{1}
	\tgBorderA{(5,0)}{white}{white}{white}{white}
	\tgBorder{(5,0)}{0}{1}{0}{1}
	\tgBorderA{(0,1)}{white}{white}{white}{white}
	\tgBorder{(0,1)}{0}{1}{0}{0}
	\tgBorderA{(1,1)}{white}{white}{white}{white}
	\tgBorder{(1,1)}{1}{0}{1}{1}
	\tgBlank{(2,1)}{white}
	\tgBlank{(3,1)}{white}
	\tgBlank{(4,1)}{white}
	\tgBlank{(5,1)}{white}
	\tgBlank{(0,2)}{white}
	\tgBorderC{(1,2)}{0}{white}{white}
	\tgBorderA{(2,2)}{white}{white}{white}{white}
	\tgBorder{(2,2)}{0}{1}{0}{1}
	\tgBorderA{(3,2)}{white}{white}{white}{white}
	\tgBorder{(3,2)}{0}{1}{0}{1}
	\tgBorderA{(4,2)}{white}{white}{white}{white}
	\tgBorder{(4,2)}{0}{1}{0}{1}
	\tgBorderA{(5,2)}{white}{white}{white}{white}
	\tgBorder{(5,2)}{0}{1}{0}{1}
	\tgBlank{(0,3)}{white}
	\tgBlank{(1,3)}{white}
	\tgBlank{(2,3)}{white}
	\tgBlank{(3,3)}{white}
	\tgBlank{(4,3)}{white}
	\tgBlank{(5,3)}{white}
	\tgRestr{(4,0)}{}
	\tgIncl{(5,0)}{}
	\tgCell[(1,1)]{(2.5,2)}{f}
	\tgCell[(0,1)]{(0,1)}{p}
\end{tangle}

==> diag/incl-restr-inverse-1.tex <==
% https://varkor.github.io/tangle/?t=W1tbXV0sW1tbMCxbXV0sWzAsW11dLFswLFtdXSxbMCxbXV0sWzAsW11dLFswLFtdXSxbMCxbXV1dLFtbMSxbMCwxLDAsMV1dLFsxLFswLDEsMCwxXV0sWzEsWzAsMSwwLDFdXSxbMSxbMCwxLDAsMV1dLFsxLFswLDEsMCwxXV0sWzEsWzAsMSwwLDFdXSxbMSxbMCwxLDAsMV1dXSxbWzAsW11dLFswLFtdXSxbMCxbXV0sWzAsW11dLFswLFtdXSxbMCxbXV0sWzAsW11dXV0sW1swLDIsMS41LFsiIl1dLFswLDMuNSwxLjUsWyJmIiwxLDFdXSxbMCwxLDEuNSxbIiJdXSxbMCw1LDEuNSxbIiJdXSxbMCw2LDEuNSxbIiJdXV0sW1swLDEsMiwiWF9wIl0sWzYsMSwwLCJYX3AiXV1d&c=F5A3A3,F5CCA3,F5F5A3,CCF5A3,A3F5A3,A3F5CC,A3F5F5,A3CCF5,A3A3F5,CCA3F5,F5A3F5,F5A3CC
\begin{tangle}{(7,3)}
	\tgBlank{(0,0)}{white}
	\tgBlank{(1,0)}{white}
	\tgBlank{(2,0)}{white}
	\tgBlank{(3,0)}{white}
	\tgBlank{(4,0)}{white}
	\tgBlank{(5,0)}{white}
	\tgBlank{(6,0)}{white}
	\tgBorderA{(0,1)}{white}{white}{white}{white}
	\tgBorder{(0,1)}{0}{1}{0}{1}
	\tgBorderA{(1,1)}{white}{white}{white}{white}
	\tgBorder{(1,1)}{0}{1}{0}{1}
	\tgBorderA{(2,1)}{white}{white}{white}{white}
	\tgBorder{(2,1)}{0}{1}{0}{1}
	\tgBorderA{(3,1)}{white}{white}{white}{white}
	\tgBorder{(3,1)}{0}{1}{0}{1}
	\tgBorderA{(4,1)}{white}{white}{white}{white}
	\tgBorder{(4,1)}{0}{1}{0}{1}
	\tgBorderA{(5,1)}{white}{white}{white}{white}
	\tgBorder{(5,1)}{0}{1}{0}{1}
	\tgBorderA{(6,1)}{white}{white}{white}{white}
	\tgBorder{(6,1)}{0}{1}{0}{1}
	\tgBlank{(0,2)}{white}
	\tgBlank{(1,2)}{white}
	\tgBlank{(2,2)}{white}
	\tgBlank{(3,2)}{white}
	\tgBlank{(4,2)}{white}
	\tgBlank{(5,2)}{white}
	\tgBlank{(6,2)}{white}
	\tgRestr{(1.5,1)}{}
	\tgCell[(1,1)]{(3,1)}{f}
	\tgIncl{(0.5,1)}{}
	\tgIncl{(4.5,1)}{}
	\tgRestr{(5.5,1)}{}
	\tgAxisLabel{(0,1.5)}{east}{X_p}
	\tgAxisLabel{(7,1.5)}{west}{X_{\incl f p}}
\end{tangle}


==> diag/incl-restr-inverse-2.tex <==
% https://varkor.github.io/tangle/?t=W1tbXV0sW1tbMCxbXV0sWzAsW11dLFswLFtdXSxbMCxbXV0sWzAsW11dLFswLFtdXSxbMCxbXV0sWzAsW11dLFswLFtdXV0sW1sxLFswLDEsMCwxXV0sWzEsWzAsMSwwLDFdXSxbMSxbMCwxLDAsMV1dLFsxLFswLDEsMCwxXV0sWzEsWzAsMSwwLDFdXSxbMSxbMCwxLDAsMV1dLFsxLFswLDEsMCwxXV0sWzEsWzAsMSwwLDFdXSxbMSxbMCwxLDAsMV1dXSxbWzAsW11dLFswLFtdXSxbMCxbXV0sWzAsW11dLFswLFtdXSxbMCxbXV0sWzAsW11dLFswLFtdXSxbMCxbXV1dXSxbWzAsNC41LDEuNSxbImciLDEsMV1dLFswLDYsMS41LFsiIl1dLFswLDcsMS41LFsiIl1dLFswLDgsMS41LFsiIl1dLFswLDMsMS41LFsiIl1dLFswLDIsMS41LFsiIl1dLFswLDEsMS41LFsiIl1dXSxbWzAsMSwyLCJYX3AiXSxbOCwxLDAsIllfe1xcaW5jbCBmIHB9Il1dXQ==&c=F5A3A3,F5CCA3,F5F5A3,CCF5A3,A3F5A3,A3F5CC,A3F5F5,A3CCF5,A3A3F5,CCA3F5,F5A3F5,F5A3CC
\begin{tangle}{(9,3)}
	\tgBlank{(0,0)}{white}
	\tgBlank{(1,0)}{white}
	\tgBlank{(2,0)}{white}
	\tgBlank{(3,0)}{white}
	\tgBlank{(4,0)}{white}
	\tgBlank{(5,0)}{white}
	\tgBlank{(6,0)}{white}
	\tgBlank{(7,0)}{white}
	\tgBlank{(8,0)}{white}
	\tgBorderA{(0,1)}{white}{white}{white}{white}
	\tgBorder{(0,1)}{0}{1}{0}{1}
	\tgBorderA{(1,1)}{white}{white}{white}{white}
	\tgBorder{(1,1)}{0}{1}{0}{1}
	\tgBorderA{(2,1)}{white}{white}{white}{white}
	\tgBorder{(2,1)}{0}{1}{0}{1}
	\tgBorderA{(3,1)}{white}{white}{white}{white}
	\tgBorder{(3,1)}{0}{1}{0}{1}
	\tgBorderA{(4,1)}{white}{white}{white}{white}
	\tgBorder{(4,1)}{0}{1}{0}{1}
	\tgBorderA{(5,1)}{white}{white}{white}{white}
	\tgBorder{(5,1)}{0}{1}{0}{1}
	\tgBorderA{(6,1)}{white}{white}{white}{white}
	\tgBorder{(6,1)}{0}{1}{0}{1}
	\tgBorderA{(7,1)}{white}{white}{white}{white}
	\tgBorder{(7,1)}{0}{1}{0}{1}
	\tgBorderA{(8,1)}{white}{white}{white}{white}
	\tgBorder{(8,1)}{0}{1}{0}{1}
	\tgBlank{(0,2)}{white}
	\tgBlank{(1,2)}{white}
	\tgBlank{(2,2)}{white}
	\tgBlank{(3,2)}{white}
	\tgBlank{(4,2)}{white}
	\tgBlank{(5,2)}{white}
	\tgBlank{(6,2)}{white}
	\tgBlank{(7,2)}{white}
	\tgBlank{(8,2)}{white}
	\tgCell[(1,1)]{(4,1)}{g}
	\tgRestr{(5.5,1)}{}
	\tgIncl{(6.5,1)}{}
	\tgRestr{(7.5,1)}{}
	\tgIncl{(2.5,1)}{}
	\tgRestr{(1.5,1)}{}
	\tgIncl{(0.5,1)}{}
	\tgAxisLabel{(0,1.5)}{east}{X_p}
	\tgAxisLabel{(9,1.5)}{west}{Y_{\incl f p}}
\end{tangle}

==> diag/incl-restr-lhs.tex <==
% https://varkor.github.io/tangle/?t=W1tbXV0sW1tbMSxbMCwxLDAsMV1dLFsxLFswLDEsMCwxXV1dXSxbWzAsMC41LDAuNSxbIiJdXSxbMCwxLjUsMC41LFsiIl1dXSxbWzAsMCwyLCJYX3AiXSxbMSwwLDAsIlhfcCJdXV0=&c=F5A3A3,F5CCA3,F5F5A3,CCF5A3,A3F5A3,A3F5CC,A3F5F5,A3CCF5,A3A3F5,CCA3F5,F5A3F5,F5A3CC
\begin{tangle}{(2,1)}
	\tgBorderA{(0,0)}{white}{white}{white}{white}
	\tgBorder{(0,0)}{0}{1}{0}{1}
	\tgBorderA{(1,0)}{white}{white}{white}{white}
	\tgBorder{(1,0)}{0}{1}{0}{1}
	\tgIncl{(0,0)}{}
	\tgRestr{(1,0)}{}
	\tgAxisLabel{(0,0.5)}{east}{X_p}
	\tgAxisLabel{(2,0.5)}{west}{X_p}
\end{tangle}

==> diag/incl-restr-rhs.tex <==
% https://varkor.github.io/tangle/?t=W1tbXV0sW1tbMSxbMCwxLDAsMV1dXV0sW10sW1swLDAsMiwiWF9wIl0sWzAsMCwwLCJYX3AiXV1d&c=F5A3A3,F5CCA3,F5F5A3,CCF5A3,A3F5A3,A3F5CC,A3F5F5,A3CCF5,A3A3F5,CCA3F5,F5A3F5,F5A3CC
\begin{tangle}{(1,1)}
	\tgBorderA{(0,0)}{white}{white}{white}{white}
	\tgBorder{(0,0)}{0}{1}{0}{1}
	\tgAxisLabel{(0,0.5)}{east}{X_p}
	\tgAxisLabel{(1,0.5)}{west}{X_p}
\end{tangle}

==> diag/restr-incl-lhs-2.tex <==
% https://varkor.github.io/tangle/?t=W1tbXV0sW1tbMSxbMCwxLDAsMV1dLFsxLFswLDEsMCwxXV0sWzEsWzAsMSwwLDFdXV1dLFtbMCwwLjUsMC41LFsiIl1dLFswLDEuNSwwLjUsWyIiXV0sWzAsMi41LDAuNSxbIiJdXV0sW1swLDAsMiwiWF9wIl0sWzIsMCwwLCJYX3AiXV1d&c=F5A3A3,F5CCA3,F5F5A3,CCF5A3,A3F5A3,A3F5CC,A3F5F5,A3CCF5,A3A3F5,CCA3F5,F5A3F5,F5A3CC
\begin{tangle}{(3,1)}
	\tgBorderA{(0,0)}{white}{white}{white}{white}
	\tgBorder{(0,0)}{0}{1}{0}{1}
	\tgBorderA{(1,0)}{white}{white}{white}{white}
	\tgBorder{(1,0)}{0}{1}{0}{1}
	\tgBorderA{(2,0)}{white}{white}{white}{white}
	\tgBorder{(2,0)}{0}{1}{0}{1}
	\tgIncl{(0,0)}{}
	\tgRestr{(1,0)}{}
	\tgIncl{(2,0)}{}
	\tgAxisLabel{(0,0.5)}{east}{X_p}
	\tgAxisLabel{(3,0.5)}{west}{X}
\end{tangle}

==> diag/restr-incl-lhs.tex <==
% https://varkor.github.io/tangle/?t=W1tbXV0sW1tbMSxbMCwxLDAsMV1dLFsxLFswLDEsMCwxXV1dXSxbWzAsMC41LDAuNSxbIiJdXSxbMCwxLjUsMC41LFsiIl1dXSxbWzAsMCwyLCJYIl0sWzEsMCwwLCJYIl1dXQ==&c=F5A3A3,F5CCA3,F5F5A3,CCF5A3,A3F5A3,A3F5CC,A3F5F5,A3CCF5,A3A3F5,CCA3F5,F5A3F5,F5A3CC
\begin{tangle}{(2,1)}
	\tgBorderA{(0,0)}{white}{white}{white}{white}
	\tgBorder{(0,0)}{0}{1}{0}{1}
	\tgBorderA{(1,0)}{white}{white}{white}{white}
	\tgBorder{(1,0)}{0}{1}{0}{1}
	\tgRestr{(0,0)}{}
	\tgIncl{(1,0)}{}
	\tgAxisLabel{(0,0.5)}{east}{X}
	\tgAxisLabel{(2,0.5)}{west}{X}
\end{tangle}

==> diag/restr-incl-rhs-2.tex <==
% https://varkor.github.io/tangle/?t=W1tbXV0sW1tbMSxbMCwxLDAsMV1dLFsxLFswLDEsMCwxXV0sWzEsWzAsMSwwLDFdXV1dLFtbMCwyLjUsMC41LFsiIl1dXSxbWzAsMCwyLCJYX3AiXSxbMiwwLDAsIlgiXV1d&c=F5A3A3,F5CCA3,F5F5A3,CCF5A3,A3F5A3,A3F5CC,A3F5F5,A3CCF5,A3A3F5,CCA3F5,F5A3F5,F5A3CC
\begin{tangle}{(3,1)}
	\tgBorderA{(0,0)}{white}{white}{white}{white}
	\tgBorder{(0,0)}{0}{1}{0}{1}
	\tgBorderA{(1,0)}{white}{white}{white}{white}
	\tgBorder{(1,0)}{0}{1}{0}{1}
	\tgBorderA{(2,0)}{white}{white}{white}{white}
	\tgBorder{(2,0)}{0}{1}{0}{1}
	\tgIncl{(2,0)}{}
	\tgAxisLabel{(0,0.5)}{east}{X_p}
	\tgAxisLabel{(3,0.5)}{west}{X}
\end{tangle}

==> diag/restr-incl-rhs.tex <==
% https://varkor.github.io/tangle/?t=W1tbXV0sW1tbMSxbMCwxLDAsMV1dXV0sW10sW1swLDAsMiwiWCJdLFswLDAsMCwiWCJdXV0=&c=F5A3A3,F5CCA3,F5F5A3,CCF5A3,A3F5A3,A3F5CC,A3F5F5,A3CCF5,A3A3F5,CCA3F5,F5A3F5,F5A3CC
\begin{tangle}{(1,1)}
	\tgBorderA{(0,0)}{white}{white}{white}{white}
	\tgBorder{(0,0)}{0}{1}{0}{1}
	\tgAxisLabel{(0,0.5)}{east}{X}
	\tgAxisLabel{(1,0.5)}{west}{X}
\end{tangle}
